ANTARES and IceCube Combined Search for Neutrino Point-like and Extended Sources in the Southern Sky

A search for point-like and extended sources of cosmic neutrinos using data collected by the ANTARES and IceCube neutrino telescopes is presented. The data set consists of all the track-like and shower-like events pointing in the direction of the Southern Sky included in the nine-year ANTARES point-source analysis, combined with the through-going track-like events used in the seven-year IceCube point-source search. The advantageous field of view of ANTARES and the large size of IceCube are exploited to improve the sensitivity in the Southern Sky by a factor $\sim$2 compared to both individual analyses. In this work, the Southern Sky is scanned for possible excesses of spatial clustering, and the positions of preselected candidate sources are investigated. In addition, special focus is given to the region around the Galactic Centre, whereby a dedicated search at the location of SgrA* is performed, and to the location of the supernova remnant RXJ 1713.7-3946. No significant evidence for cosmic neutrino sources is found and upper limits on the flux from the various searches are presented.

==> author_list_antares.tex <==
%updated to 04/12/2019

\author[1,2]{A.~Albert}
\author[3]{M.~Andr\'e}
\author[4]{M.~Anghinolfi}
\author[5]{G.~Anton}
\author[6]{M.~Ardid}
\author[7]{J.-J.~Aubert}
\author[8]{J.~Aublin}
\author[8]{B.~Baret}
\author[9]{S.~Basa}
\author[10]{B.~Belhorma}
\author[7]{V.~Bertin}
\author[11]{S.~Biagi}
\author[5]{M.~Bissinger}
\author[12]{J.~Boumaaza}
\author[8]{S.~Bourret}
\author[13]{M.~Bouta}
\author[14]{M.C.~Bouwhuis}
\author[15]{H.~Br\^{a}nza\c{s}}
\author[14,16]{R.~Bruijn}
\author[7]{J.~Brunner}
\author[7]{J.~Busto}
\author[17,18]{A.~Capone}
\author[15]{L.~Caramete}
\author[7]{J.~Carr}
\author[17,18,19]{S.~Celli}
\author[20]{M.~Chabab}
\author[8]{T. N.~Chau}
\author[12]{R.~Cherkaoui El Moursli}
\author[21]{T.~Chiarusi}
\author[22]{M.~Circella}
\author[8]{A.~Coleiro}
\author[8,23]{M.~Colomer}
\author[11]{R.~Coniglione}
\author[7]{H.~Costantini}
\author[7]{P.~Coyle}
\author[8]{A.~Creusot}
\author[24]{A.~F.~D\'\i{}az}
\author[8]{G.~de~Wasseige}
\author[25]{A.~Deschamps}
\author[11]{C.~Distefano}
\author[17,18]{I.~Di~Palma}
\author[4,26]{A.~Domi}
\author[8,27]{C.~Donzaud}
\author[7]{D.~Dornic}
\author[1,2]{D.~Drouhin}
\author[5]{T.~Eberl}
\author[13]{I.~El Bojaddaini}
\author[12]{N.~El~Khayati}
\author[28]{D.~Els\"asser}
\author[5,7]{A.~Enzenh\"ofer}
\author[12]{A.~Ettahiri}
\author[12]{F.~Fassi}
\author[17,18]{P.~Fermani}
\author[11]{G.~Ferrara}
\author[21,29]{F.~Filippini}
\author[8,29]{L.~Fusco}
\author[30,8]{P.~Gay}
\author[31]{H.~Glotin}
\author[23]{R.~Gozzini}
\author[1]{R.~Gracia~Ruiz}
\author[5]{K.~Graf}
\author[4,26]{C.~Guidi}
\author[5]{S.~Hallmann}
\author[32]{H.~van~Haren}
\author[14]{A.J.~Heijboer}
\author[25]{Y.~Hello}
\author[23]{J.J. ~Hern\'andez-Rey}
\author[5]{J.~H\"o{\ss}l}
\author[5]{J.~Hofest\"adt}
\author[23]{G.~Illuminati}
\author[33]{C.~W.~James}
\author[14,34]{M. de~Jong}
\author[14]{P. de~Jong}
\author[14]{M.~Jongen}
\author[28]{M.~Kadler}
\author[5]{O.~Kalekin}
\author[5]{U.~Katz}
\author[23]{N.R.~Khan-Chowdhury}
\author[8,35]{A.~Kouchner}
\author[28]{M.~Kreter}
\author[36]{I.~Kreykenbohm}
\author[4,37]{V.~Kulikovskiy}
\author[5]{R.~Lahmann}
\author[8]{R.~Le~Breton}
\author[38]{D. ~Lef\`evre}
\author[39]{E.~Leonora}
\author[21,29]{G.~Levi}
\author[7]{M.~Lincetto}
\author[40]{D.~Lopez-Coto}
\author[41,8]{S.~Loucatos}
\author[7]{G.~Maggi}
\author[23]{J.~Manczak}
\author[9]{M.~Marcelin}
\author[21,29]{A.~Margiotta}
\author[42,43]{A.~Marinelli}
\author[6]{J.A.~Mart\'inez-Mora}
\author[44,45]{R.~Mele}
\author[14,16]{K.~Melis}
\author[44]{P.~Migliozzi}
\author[5]{M.~Moser}
\author[13]{A.~Moussa}
\author[14]{R.~Muller}
\author[14]{L.~Nauta}
\author[40]{S.~Navas}
\author[9]{E.~Nezri}
\author[8]{C.~Nielsen}
\author[7,9]{A.~Nu\~nez-Casti\~neyra}
\author[14]{B.~O'Fearraigh}
\author[1]{M.~Organokov}
\author[15]{G.E.~P\u{a}v\u{a}la\c{s}}
\author[21,29]{C.~Pellegrino}
\author[7]{M.~Perrin-Terrin}
\author[11]{P.~Piattelli}
\author[6]{C.~Poir\`e}
\author[15]{V.~Popa}
\author[1]{T.~Pradier}
\author[7]{L.~Quinn}
\author[39]{N.~Randazzo}
\author[11]{G.~Riccobene}
\author[22]{A.~S\'anchez-Losa}
\author[20]{A.~Salah-Eddine}
\author[14,34]{D. F. E.~Samtleben}
\author[4,26]{M.~Sanguineti}
\author[11]{P.~Sapienza}
\author[41]{F.~Sch\"ussler}
\author[21,29]{M.~Spurio}
\author[41]{Th.~Stolarczyk}
\author[14]{B.~Strandberg}
\author[4,26]{M.~Taiuti}
\author[12]{Y.~Tayalati}
\author[23]{T.~Thakore}
\author[33]{S.J.~Tingay}
\author[11]{A.~Trovato}
\author[41,8]{B.~Vallage}
\author[8,35]{V.~Van~Elewyck}
\author[21,29,8]{F.~Versari}
\author[11]{S.~Viola}
\author[44,45]{D.~Vivolo}
\author[36]{J.~Wilms}
\author[7]{D.~Zaborov}
\author[17,18]{A.~Zegarelli}
\author[23]{J.D.~Zornoza}
\author[23]{and J.~Z\'u\~{n}iga}

\affil[1]{\scriptsize{Universit\'e de Strasbourg, CNRS,  IPHC UMR 7178, F-67000 Strasbourg, France}}
\affil[2]{\scriptsize{Universit\'e de Haute Alsace, F-68200 Mulhouse, France}}
\affil[3]{\scriptsize{Technical University of Catalonia, Laboratory of Applied Bioacoustics, Rambla Exposici\'o, 08800 Vilanova i la Geltr\'u, Barcelona, Spain}}
\affil[4]{\scriptsize{INFN - Sezione di Genova, Via Dodecaneso 33, 16146 Genova, Italy}}
\affil[5]{\scriptsize{Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, 91058 Erlangen, Germany}}
\affil[6]{\scriptsize{Institut d'Investigaci\'o per a la Gesti\'o Integrada de les Zones Costaneres (IGIC) - Universitat Polit\`ecnica de Val\`encia. C/  Paranimf 1, 46730 Gandia, Spain}}
\affil[7]{\scriptsize{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}}
\affil[8]{\scriptsize{APC, Univ Paris Diderot, CNRS/IN2P3, CEA/Irfu, Obs de Paris, Sorbonne Paris Cit\'e, France}}
\affil[9]{\scriptsize{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France }}
\affil[10]{\scriptsize{National Center for Energy Sciences and Nuclear Techniques, B.P.1382, R. P.10001 Rabat, Morocco}}
\affil[11]{\scriptsize{INFN - Laboratori Nazionali del Sud (LNS), Via S. Sofia 62, 95123 Catania, Italy}}
\affil[12]{\scriptsize{University Mohammed V in Rabat, Faculty of Sciences, 4 av. Ibn Battouta, B.P. 1014, R.P. 10000}}
\affil[13]{\scriptsize{University Mohammed I, Laboratory of Physics of Matter and Radiations, B.P.717, Oujda 6000, Morocco}}
\affil[14]{\scriptsize{Nikhef, Science Park,  Amsterdam, The Netherlands}}
\affil[15]{\scriptsize{Institute of Space Science, RO-077125 Bucharest, M\u{a}gurele, Romania}}
\affil[16]{\scriptsize{Universiteit van Amsterdam, Instituut voor Hoge-Energie Fysica, Science Park 105, 1098 XG Amsterdam, The Netherlands}}
\affil[17]{\scriptsize{INFN - Sezione di Roma, P.le Aldo Moro 2, 00185 Roma, Italy}}
\affil[18]{\scriptsize{Dipartimento di Fisica dell'Universit\`a La Sapienza, P.le Aldo Moro 2, 00185 Roma, Italy}}
\affil[19]{\scriptsize{Gran Sasso Science Institute, Viale Francesco Crispi 7, 00167 L'Aquila, Italy}}
\affil[20]{\scriptsize{LPHEA, Faculty of Science - Semlali, Cadi Ayyad University, P.O.B. 2390, Marrakech, Morocco.}}
\affil[21]{\scriptsize{INFN - Sezione di Bologna, Viale Berti-Pichat 6/2, 40127 Bologna, Italy}}
\affil[22]{\scriptsize{INFN - Sezione di Bari, Via E. Orabona 4, 70126 Bari, Italy}}
\affil[23]{\scriptsize{IFIC - Instituto de F\'isica Corpuscular (CSIC - Universitat de Val\`encia) c/ Catedr\'atico Jos\'e Beltr\'an, 2 E-46980 Paterna, Valencia, Spain}}
\affil[24]{\scriptsize{Department of Computer Architecture and Technology/CITIC, University of Granada, 18071 Granada, Spain}}
\affil[25]{\scriptsize{G\'eoazur, UCA, CNRS, IRD, Observatoire de la C\^ote d'Azur, Sophia Antipolis, France}}
\affil[26]{\scriptsize{Dipartimento di Fisica dell'Universit\`a, Via Dodecaneso 33, 16146 Genova, Italy}}
\affil[27]{\scriptsize{Universit\'e Paris-Sud, 91405 Orsay Cedex, France}}
\affil[28]{\scriptsize{Institut f\"ur Theoretische Physik und Astrophysik, Universit\"at W\"urzburg, Emil-Fischer Str. 31, 97074 W\"urzburg, Germany}}
\affil[29]{\scriptsize{Dipartimento di Fisica e Astronomia dell'Universit\`a, Viale Berti Pichat 6/2, 40127 Bologna, Italy}}
\affil[30]{\scriptsize{Laboratoire de Physique Corpusculaire, Clermont Universit\'e, Universit\'e Blaise Pascal, CNRS/IN2P3, BP 10448, F-63000 Clermont-Ferrand, France}}
\affil[31]{\scriptsize{LIS, UMR Universit\'e de Toulon, Aix Marseille Universit\'e, CNRS, 83041 Toulon, France}}
\affil[32]{\scriptsize{Royal Netherlands Institute for Sea Research (NIOZ) and Utrecht University, Landsdiep 4, 1797 SZ 't Horntje (Texel), the Netherlands}}
\affil[33]{\scriptsize{International Centre for Radio Astronomy Research - Curtin University, Bentley, WA 6102, Australia}}
\affil[34]{\scriptsize{Huygens-Kamerlingh Onnes Laboratorium, Universiteit Leiden, The Netherlands}}
\affil[35]{\scriptsize{Institut Universitaire de France, 75005 Paris, France}}
\affil[36]{\scriptsize{Dr. Remeis-Sternwarte and ECAP, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg,  Sternwartstr. 7, 96049 Bamberg, Germany}}
\affil[37]{\scriptsize{Moscow State University, Skobeltsyn Institute of Nuclear Physics, Leninskie gory, 119991 Moscow, Russia}}
\affil[38]{\scriptsize{Mediterranean Institute of Oceanography (MIO), Aix-Marseille University, 13288, Marseille, Cedex 9, France; Universit\'e du Sud Toulon-Var,  CNRS-INSU/IRD UM 110, 83957, La Garde Cedex, France}}
\affil[39]{\scriptsize{INFN - Sezione di Catania, Via S. Sofia 64, 95123 Catania, Italy}}
\affil[40]{\scriptsize{Dpto. de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., University of Granada, 18071 Granada, Spain}}
\affil[41]{\scriptsize{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}}
\affil[42]{\scriptsize{INFN - Sezione di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}}
\affil[43]{\scriptsize{Dipartimento di Fisica dell'Universit\`a, Largo B. Pontecorvo 3, 56127 Pisa, Italy}}
\affil[44]{\scriptsize{INFN - Sezione di Napoli, Via Cintia 80126 Napoli, Italy}}
\affil[45]{\scriptsize{Dipartimento di Fisica dell'Universit\`a Federico II di Napoli, Via Cintia 80126, Napoli, Italy}}


==> author_list_icecube.tex <==
%updated to 16/12/2019

\author[61]{M. G. Aartsen}
\author[100]{M. Ackermann}
\author[61]{J. Adams}
\author[57]{J. A. Aguilar}
\author[65]{M. Ahlers}
\author[91]{M. Ahrens}
\author[71]{C. Alispach}
\author[82]{K. Andeen}
\author[97]{T. Anderson}
\author[57]{I. Ansseau}
\author[69]{G. Anton}
\author[59]{C. Arg{\"u}elles}
\author[46]{J. Auffenberg}
\author[59]{S. Axani}
\author[46]{P. Backes}
\author[61]{H. Bagherpour}
\author[88]{X. Bai}
\author[74]{A. Balagopal V.}
\author[71]{A. Barbano}
\author[73]{S. W. Barwick}
\author[100]{B. Bastian}
\author[81]{V. Baum}
\author[57]{S. Baur}
\author[53]{R. Bay}
\author[63,64]{J. J. Beatty}
\author[99]{K.-H. Becker}
\author[56]{J. Becker Tjus}
\author[90]{S. BenZvi}
\author[62]{D. Berley}
\author[100,a]{E. Bernardini}
\author[75,b]{D. Z. Besson}
\author[53,54]{G. Binder}
\author[99]{D. Bindig}
\author[62]{E. Blaufuss}
\author[100]{S. Blot}
\author[91]{C. Bohm}
\author[81]{S. B{\"o}ser}
\author[98]{O. Botner}
\author[46]{J. B{\"o}ttcher}
\author[65]{E. Bourbeau}
\author[80]{J. Bourbeau}
\author[100]{F. Bradascio}
\author[80]{J. Braun}
\author[71]{S. Bron}
\author[100]{J. Brostean-Kaiser}
\author[98]{A. Burgman}
\author[46]{J. Buscher}
\author[83]{R. S. Busse}
\author[71]{T. Carver}
\author[51]{C. Chen}
\author[62]{E. Cheung}
\author[80]{D. Chirkin}
\author[93]{S. Choi}
\author[76]{K. Clark}
\author[83]{L. Classen}
\author[84]{A. Coleman}
\author[59]{G. H. Collin}
\author[59]{J. M. Conrad}
\author[58]{P. Coppin}
\author[58]{P. Correa}
\author[96,97]{D. F. Cowen}
\author[90]{R. Cross}
\author[51]{P. Dave}
\author[58]{C. De Clercq}
\author[97]{J. J. DeLaunay}
\author[84]{H. Dembinski}
\author[91]{K. Deoskar}
\author[72]{S. De Ridder}
\author[80]{P. Desiati}
\author[58]{K. D. de Vries}
\author[58]{G. de Wasseige}
\author[55]{M. de With}
\author[67]{T. DeYoung}
\author[59]{A. Diaz}
\author[80]{J. C. D{\'\i}az-V{\'e}lez}
\author[74]{H. Dujmovic}
\author[97]{M. Dunkman}
\author[88]{E. Dvorak}
\author[80]{B. Eberhardt}
\author[81]{T. Ehrhardt}
\author[97]{P. Eller}
\author[74]{R. Engel}
\author[84]{P. A. Evenson}
\author[80]{S. Fahey}
\author[52]{A. R. Fazely}
\author[62]{J. Felde}
\author[53]{K. Filimonov}
\author[91]{C. Finley}
\author[96]{D. Fox}
\author[100]{A. Franckowiak}
\author[62]{E. Friedman}
\author[81]{A. Fritz}
\author[84]{T. K. Gaisser}
\author[79]{J. Gallagher}
\author[46]{E. Ganster}
\author[100]{S. Garrappa}
\author[54]{L. Gerhardt}
\author[80]{K. Ghorbani}
\author[70]{T. Glauch}
\author[69]{T. Gl{\"u}senkamp}
\author[54]{A. Goldschmidt}
\author[84]{J. G. Gonzalez}
\author[67]{D. Grant}
\author[97]{T. Gr{\'e}goire}
\author[80]{Z. Griffith}
\author[90]{S. Griswold}
\author[46]{M. G{\"u}nder}
\author[56]{M. G{\"u}nd{\"u}z}
\author[46]{C. Haack}
\author[98]{A. Hallgren}
\author[67]{R. Halliday}
\author[46]{L. Halve}
\author[80]{F. Halzen}
\author[80]{K. Hanson}
\author[74]{A. Haungs}
\author[55]{D. Hebecker}
\author[57]{D. Heereman}
\author[46]{P. Heix}
\author[99]{K. Helbing}
\author[62]{R. Hellauer}
\author[70]{F. Henningsen}
\author[99]{S. Hickford}
\author[68]{J. Hignight}
\author[47]{G. C. Hill}
\author[62]{K. D. Hoffman}
\author[99]{R. Hoffmann}
\author[66]{T. Hoinka}
\author[80]{B. Hokanson-Fasig}
\author[80,c]{K. Hoshina}
\author[97]{F. Huang}
\author[70]{M. Huber}
\author[74,100]{T. Huber}
\author[91]{K. Hultqvist}
\author[66]{M. H{\"u}nnefeld}
\author[80]{R. Hussain}
\author[93]{S. In}
\author[57]{N. Iovine}
\author[60]{A. Ishihara}
\author[91]{M. Jansson}
\author[50]{G. S. Japaridze}
\author[93]{M. Jeong}
\author[80]{K. Jero}
\author[49]{B. J. P. Jones}
\author[46]{F. Jonske}
\author[46]{R. Joppe}
\author[74]{D. Kang}
\author[93]{W. Kang}
\author[83]{A. Kappes}
\author[81]{D. Kappesser}
\author[100]{T. Karg}
\author[70]{M. Karl}
\author[80]{A. Karle}
\author[69]{U. Katz}
\author[80]{M. Kauer}
\author[80]{J. L. Kelley}
\author[80]{A. Kheirandish}
\author[93]{J. Kim}
\author[100]{T. Kintscher}
\author[92]{J. Kiryluk}
\author[69]{T. Kittler}
\author[53,54]{S. R. Klein}
\author[84]{R. Koirala}
\author[55]{H. Kolanoski}
\author[81]{L. K{\"o}pke}
\author[67]{C. Kopper}
\author[95]{S. Kopper}
\author[65]{D. J. Koskinen}
\author[55,100]{M. Kowalski}
\author[70]{K. Krings}
\author[81]{G. Kr{\"u}ckl}
\author[68]{N. Kulacz}
\author[87]{N. Kurahashi}
\author[47]{A. Kyriacou}
\author[97]{J. L. Lanfranchi}
\author[62]{M. J. Larson}
\author[99]{F. Lauber}
\author[80]{J. P. Lazar}
\author[80]{K. Leonard}
\author[74]{A. Leszczy{\'n}ska}
\author[46]{M. Leuermann}
\author[80]{Q. R. Liu}
\author[81]{E. Lohfink}
\author[83]{C. J. Lozano Mariscal}
\author[60]{L. Lu}
\author[71]{F. Lucarelli}
\author[58]{J. L{\"u}nemann}
\author[80]{W. Luszczak}
\author[53,54]{Y. Lyu}
\author[100]{W. Y. Ma}
\author[89]{J. Madsen}
\author[58]{G. Maggi}
\author[67]{K. B. M. Mahn}
\author[60]{Y. Makino}
\author[46]{P. Mallik}
\author[80]{K. Mallot}
\author[80]{S. Mancina}
\author[57]{I. C. Mari{\c{s}}}
\author[85]{R. Maruyama}
\author[60]{K. Mase}
\author[62]{R. Maunu}
\author[78]{F. McNally}
\author[80]{K. Meagher}
\author[65]{M. Medici}
\author[64]{A. Medina}
\author[66]{M. Meier}
\author[70]{S. Meighen-Berger}
\author[80]{G. Merino}
\author[57]{T. Meures}
\author[67]{J. Micallef}
\author[57]{D. Mockler}
\author[81]{G. Moment{\'e}}
\author[71]{T. Montaruli}
\author[68]{R. W. Moore}
\author[80]{R. Morse}
\author[59]{M. Moulai}
\author[46]{P. Muth}
\author[60]{R. Nagai}
\author[99]{U. Naumann}
\author[67]{G. Neer}
\author[70]{H. Niederhausen}
\author[67]{M. U. Nisa}
\author[67]{S. C. Nowicki}
\author[54]{D. R. Nygren}
\author[99]{A. Obertacke Pollmann}
\author[74]{M. Oehler}
\author[62]{A. Olivas}
\author[57]{A. O'Murchadha}
\author[91]{E. O'Sullivan}
\author[53,54]{T. Palczewski}
\author[84]{H. Pandya}
\author[97]{D. V. Pankova}
\author[80]{N. Park}
\author[81]{P. Peiffer}
\author[98]{C. P{\'e}rez de los Heros}
\author[46]{S. Philippen}
\author[66]{D. Pieloth}
\author[99]{S. Pieper}
\author[57]{E. Pinat}
\author[80]{A. Pizzuto}
\author[82]{M. Plum}
\author[72]{A. Porcelli}
\author[53]{P. B. Price}
\author[54]{G. T. Przybylski}
\author[57]{C. Raab}
\author[61]{A. Raissi}
\author[65]{M. Rameez}
\author[100]{L. Rauch}
\author[48]{K. Rawlins}
\author[70]{I. C. Rea}
\author[46]{R. Reimann}
\author[87]{B. Relethford}
\author[74]{M. Renschler}
\author[57]{G. Renzi}
\author[70]{E. Resconi}
\author[66]{W. Rhode}
\author[87]{M. Richman}
\author[54]{S. Robertson}
\author[46]{M. Rongen}
\author[93]{C. Rott}
\author[66]{T. Ruhe}
\author[72]{D. Ryckbosch}
\author[67]{D. Rysewyk}
\author[80]{I. Safa}
\author[67]{S. E. Sanchez Herrera}
\author[66]{A. Sandrock}
\author[81]{J. Sandroos}
\author[95]{M. Santander}
\author[86]{S. Sarkar}
\author[68]{S. Sarkar}
\author[100]{K. Satalecka}
\author[46]{M. Schaufel}
\author[74]{H. Schieler}
\author[66]{P. Schlunder}
\author[62]{T. Schmidt}
\author[80]{A. Schneider}
\author[69]{J. Schneider}
\author[74,84]{F. G. Schr{\"o}der}
\author[46]{L. Schumacher}
\author[87]{S. Sclafani}
\author[84]{D. Seckel}
\author[89]{S. Seunarine}
\author[46]{S. Shefali}
\author[80]{M. Silva}
\author[80]{R. Snihur}
\author[66]{J. Soedingrekso}
\author[84]{D. Soldin}
\author[62]{M. Song}
\author[89]{G. M. Spiczak}
\author[100]{C. Spiering}
\author[100]{J. Stachurska}
\author[64]{M. Stamatikos}
\author[84]{T. Stanev}
\author[100]{R. Stein}
\author[46]{J. Stettner}
\author[81]{A. Steuer}
\author[54]{T. Stezelberger}
\author[54]{R. G. Stokstad}
\author[60]{A. St{\"o}{\ss}l}
\author[100]{N. L. Strotjohann}
\author[46]{T. St{\"u}rwald}
\author[65]{T. Stuttard}
\author[62]{G. W. Sullivan}
\author[51]{I. Taboada}
\author[56]{F. Tenholt}
\author[52]{S. Ter-Antonyan}
\author[100]{A. Terliuk}
\author[84]{S. Tilav}
\author[67]{K. Tollefson}
\author[56]{L. Tomankova}
\author[94]{C. T{\"o}nnis}
\author[57]{S. Toscano}
\author[80]{D. Tosi}
\author[100]{A. Trettin}
\author[69]{M. Tselengidou}
\author[51]{C. F. Tung}
\author[70]{A. Turcati}
\author[74]{R. Turcotte}
\author[97]{C. F. Turley}
\author[80]{B. Ty}
\author[98]{E. Unger}
\author[83]{M. A. Unland Elorrieta}
\author[100]{M. Usner}
\author[80]{J. Vandenbroucke}
\author[72]{W. Van Driessche}
\author[80]{D. van Eijk}
\author[58]{N. van Eijndhoven}
\author[100]{J. van Santen}
\author[72]{S. Verpoest}
\author[72]{M. Vraeghe}
\author[91]{C. Walck}
\author[47]{A. Wallace}
\author[46]{M. Wallraff}
\author[80]{N. Wandkowsky}
\author[49]{T. B. Watson}
\author[68]{C. Weaver}
\author[74]{A. Weindl}
\author[97]{M. J. Weiss}
\author[81]{J. Weldert}
\author[80]{C. Wendt}
\author[80]{J. Werthebach}
\author[47]{B. J. Whelan}
\author[77]{N. Whitehorn}
\author[81]{K. Wiebe}
\author[46]{C. H. Wiebusch}
\author[80]{L. Wille}
\author[95]{D. R. Williams}
\author[87]{L. Wills}
\author[70]{M. Wolf}
\author[80]{J. Wood}
\author[68]{T. R. Wood}
\author[53]{K. Woschnagg}
\author[69]{G. Wrede}
\author[80]{D. L. Xu}
\author[52]{X. W. Xu}
\author[92]{Y. Xu}
\author[68]{J. P. Yanez}
\author[73]{G. Yodh}
\author[60]{S. Yoshida}
\author[80]{T. Yuan}
\author[46]{M. Z{\"o}cklein}

\affil[46]{\scriptsize{III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany}}
\affil[47]{\scriptsize{Department of Physics, University of Adelaide, Adelaide, 5005, Australia}}
\affil[48]{\scriptsize{Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA}}
\affil[49]{\scriptsize{Dept. of Physics, University of Texas at Arlington, 502 Yates St., Science Hall Rm 108, Box 19059, Arlington, TX 76019, USA}}
\affil[50]{\scriptsize{CTSPS, Clark-Atlanta University, Atlanta, GA 30314, USA}}
\affil[51]{\scriptsize{School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA}}
\affil[52]{\scriptsize{Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA}}
\affil[53]{\scriptsize{Dept. of Physics, University of California, Berkeley, CA 94720, USA}}
\affil[54]{\scriptsize{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}}
\affil[55]{\scriptsize{Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany}}
\affil[56]{\scriptsize{Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany}}
\affil[57]{\scriptsize{Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium}}
\affil[58]{\scriptsize{Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium}}
\affil[59]{\scriptsize{Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}}
\affil[60]{\scriptsize{Dept. of Physics and Institute for Global Prominent Research, Chiba University, Chiba 263-8522, Japan}}
\affil[61]{\scriptsize{Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand}}
\affil[62]{\scriptsize{Dept. of Physics, University of Maryland, College Park, MD 20742, USA}}
\affil[63]{\scriptsize{Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA}}
\affil[64]{\scriptsize{Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA}}
\affil[65]{\scriptsize{Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark}}
\affil[66]{\scriptsize{Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany}}
\affil[67]{\scriptsize{Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}}
\affil[68]{\scriptsize{Dept. of Physics, University of Alberta, Edmonton, Alberta, Canada T6G 2E1}}
\affil[69]{\scriptsize{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany}}
\affil[70]{\scriptsize{Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany}}
\affil[71]{\scriptsize{D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland}}
\affil[72]{\scriptsize{Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium}}
\affil[73]{\scriptsize{Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA}}
\affil[74]{\scriptsize{Karlsruhe Institute of Technology, Institut f{\"u}r Kernphysik, D-76021 Karlsruhe, Germany}}
\affil[75]{\scriptsize{Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA}}
\affil[76]{\scriptsize{SNOLAB, 1039 Regional Road 24, Creighton Mine 9, Lively, ON, Canada P3Y 1N2}}
\affil[77]{\scriptsize{Department of Physics and Astronomy, UCLA, Los Angeles, CA 90095, USA}}
\affil[78]{\scriptsize{Department of Physics, Mercer University, Macon, GA 31207-0001, USA}}
\affil[79]{\scriptsize{Dept. of Astronomy, University of Wisconsin, Madison, WI 53706, USA}}
\affil[80]{\scriptsize{Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin, Madison, WI 53706, USA}}
\affil[81]{\scriptsize{Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany}}
\affil[82]{\scriptsize{Department of Physics, Marquette University, Milwaukee, WI, 53201, USA}}
\affil[83]{\scriptsize{Institut f{\"u}r Kernphysik, Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany}}
\affil[84]{\scriptsize{Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA}}
\affil[85]{\scriptsize{Dept. of Physics, Yale University, New Haven, CT 06520, USA}}
\affil[86]{\scriptsize{Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, UK}}
\affil[87]{\scriptsize{Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA}}
\affil[88]{\scriptsize{Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}}
\affil[89]{\scriptsize{Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA}}
\affil[90]{\scriptsize{Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA}}
\affil[91]{\scriptsize{Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden}}
\affil[92]{\scriptsize{Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA}}
\affil[93]{\scriptsize{Dept. of Physics, Sungkyunkwan University, Suwon 16419, Korea}}
\affil[94]{\scriptsize{Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Korea}}
\affil[95]{\scriptsize{Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}}
\affil[96]{\scriptsize{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}}
\affil[97]{\scriptsize{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}}
\affil[98]{\scriptsize{Dept. of Physics and Astronomy, Uppsala University, Box 516, S-75120 Uppsala, Sweden}}
\affil[99]{\scriptsize{Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany}}
\affil[100]{\scriptsize{DESY, D-15738 Zeuthen, Germany}}
\affil[a]{\scriptsize{also at Universit{\`a} di Padova, I-35131 Padova, Italy}}
\affil[b]{\scriptsize{also at National Research Nuclear University, Moscow Engineering Physics Institute (MEPhI), Moscow 115409, Russia}}
\affil[c]{\scriptsize{Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan}}




